Rethinking Local Learning: A Cheaper and Faster Recipe for LLM Post-Training

LLM post-training typically propagates task gradients through the full depth of the model. Although this end-to-end structure is simple and general, it couples task adaptation to full-depth activation storage, long-range backward dependencies and direct task-gradient access to pretrained representations. We argue that this full-depth backward coupling can be unnecessarily expensive and intrusive, particularly when post-training supervision is much narrower than pre-training. To this end, we propose \textbf{LoPT}: Local-Learning Post-Training, a simple post-training strategy that makes gradient reach an explicit design choice. LoPT places a single gradient boundary at the transformer midpoint: the second-half block learns from the task objective, while the first-half block is updated by a lightweight feature-reconstruction objective to preserve useful representations and maintain interface compatibility. LoPT shortens the task-induced backward path while limiting direct interference from narrow task gradients on early-layer representations. Extensive experiments demonstrate that LoPT achieves competitive performance with lower memory cost, higher training efficiency and better retention of pretrained capabilities. Our code is available at: https://github.com/HumyuShi/LoPT

==> checklist.tex <==
% NeurIPS Paper Checklist

\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    % \item[] Justification: Within the single-run settings reported, the main claims are supported by the results in Section~\ref{sec:results}. The cross-configuration SFT pattern is \shy{summarized in Table~\ref{tab:sft_quality_efficiency} and Appendix~\ref{app:full_sft}}; efficiency claims are supported by the main-text efficiency tables and \shy{Appendix~\ref{app:extended_efficiency}}; ablation claims by \shy{Tables~\ref{tab:front14_perturb}, \ref{tab:k4_ablation}, and \ref{tab:freeze_grpo}}; and GRPO and 32B claims are presented as limited checks rather than broad guarantees. Small deltas are treated as near parity rather than strong improvements.
    \item[] Justification: Within the three-seed settings reported, the main claims are supported by the results in Section~\ref{sec:results}. The cross-configuration SFT pattern is summarized in Table~\ref{tab:sft_quality_efficiency} and Appendix~\ref{app:full_sft}; efficiency claims are supported by the main-text efficiency tables and Appendix~\ref{app:extended_efficiency}; ablation claims by Tables~\ref{tab:front14_perturb}, \ref{tab:k4_ablation}, and \ref{tab:freeze_grpo}; and GRPO and 32B claims are presented as limited checks rather than broad guarantees. Small deltas are treated as near parity rather than strong improvements.

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: Appendix~\ref{sec:limitations} discusses two main scope limitations: the main quality sweep focuses on 4B--8B models with a limited 32B GRPO sanity check, and the split-design study compares the midpoint \(k{=}2\) setting with only one finer \(k{=}4\) variant.

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (or correct) proof?
    \item[] Answer: \answerYes{}
    \item[] Justification: Appendix~\ref{app:theory} states the local assumptions used in the theoretical analysis and provides proofs for the lemmas, propositions, and corollaries.

\item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper?
    \item[] Answer: \answerYes{}
    \item[] Justification: Section~\ref{sec:setup} reports the main hyperparameters, model specifications, dataset details, and evaluation protocols needed to interpret the reported results. Appendix~\ref{app:grpo_details}, Appendix~\ref{app:exact_impl}, and Appendix~\ref{app:metrics} provide GRPO-specific details, exact configuration items to pin, and exact metric conventions. Code and configs will be released upon acceptance.

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results?
    \item[] Answer: \answerNo{}
    \item[] Justification: Code and configs will be released upon acceptance. All training datasets (Alpaca, Tulu-3, Magpie, MetaMathQA, GSM8K, and NuminaMath) and evaluation benchmarks are publicly available.

\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: Training details in Section~\ref{sec:setup}; evaluation setup with exact metric keys in Appendix~\ref{app:metrics}; hardware and compute budget in Appendix~\ref{app:compute}.

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{}
    \item[] Justification: Main results are averaged over three independent runs with different random seeds, but we do not report full error bars or confidence intervals for every table. We therefore interpret small deltas cautiously and focus on consistent trends and larger effect sizes.

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources needed to reproduce the experiment?
    \item[] Answer: \answerYes{}
    \item[] Justification: Hardware, software details, and the total compute budget ($\sim$3,400 A100-hours) are reported in Appendix~\ref{app:compute}, which distinguishes profiling costs from full training and evaluation costs.

\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics?
    \item[] Answer: \answerYes{}
    \item[] Justification: This work proposes a training methodology for publicly available models and datasets. It does not raise ethical concerns beyond those inherent to general-purpose language model training.

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work?
    \item[] Answer: \answerYes{}
    \item[] Justification: A potential positive impact is that the method may reduce hardware barriers in some profiled settings by lowering training memory requirements. A potential negative impact is that cheaper post-training could also lower the cost of adapting capable language models for harmful or low-quality uses. These risks are inherited from the underlying models and datasets rather than being specific to LoPT, and we do not release new data or deploy a new model.

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible disclosure of data with personal or offensive content?
    \item[] Answer: \answerNA{}
    \item[] Justification: This work uses established public datasets and pre-trained models; no new data collection or model deployment is performed.

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets used in the paper properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: All models and datasets are properly cited. Qwen models are Apache-2.0 licensed; Llama models are under the Meta Llama license; all SFT datasets and benchmarks are publicly available under their respective licenses.

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}
    \item[] Justification: No new datasets or pre-trained models are released in this paper. Code and configs will be released upon acceptance.

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots?
    \item[] Answer: \answerNA{}
    \item[] Justification: No crowdsourcing or human subject research is involved.

\item {\bf Institutional Review Board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether consent was obtained or waived, and any potential risks of study participation?
    \item[] Answer: \answerNA{}
    \item[] Justification: No human subject research is involved.

\end{enumerate}


==> sections/limitations.tex <==
% ===========================================================================
% 6. LIMITATIONS
% ===========================================================================
\FloatBarrier
\section{Limitations}
\label{sec:limitations}

Our study has several limitations. First, we use a fixed two-block midpoint split. A preliminary four-block variant did not improve in our setup, but the best split location and number of blocks remain open. Second, the main quality sweep covers 4B--8B models, with only one 32B GRPO sanity check rather than a broad scaling study. Third, our mechanism evidence comes from downstream ablations rather than direct representation diagnostics such as CKA, hidden-state drift, or layerwise parameter movement. Fourth, all training results are single-run, so small deltas, especially in GRPO, should be treated cautiously. Finally, we use one main auxiliary objective and one auxiliary weight; broader searches over local objectives and split policies remain future work.
